Entire Space Multi-Task Model: An Effective Approach for Estimating Post-Click Conversion Rate

Estimating post-click conversion rate (CVR) accurately is crucial for ranking systems in industrial applications such as recommendation and advertising. Conventional CVR modeling applies popular deep learning methods and achieves state-of-the-art performance. However it encounters several task-specific problems in practice, making CVR modeling challenging. For example, conventional CVR models are trained with samples of clicked impressions while utilized to make inference on the entire space with samples of all impressions. This causes a sample selection bias problem. Besides, there exists an extreme data sparsity problem, making the model fitting rather difficult. In this paper, we model CVR in a brand-new perspective by making good use of sequential pattern of user actions, i.e., impression -> click -> conversion. The proposed Entire Space Multi-task Model (ESMM) can eliminate the two problems simultaneously by i) modeling CVR directly over the entire space, ii) employing a feature representation transfer learning strategy. Experiments on dataset gathered from Taobao's recommender system demonstrate that ESMM significantly outperforms competitive methods. We also release a sampling version of this dataset to enable future research. To the best of our knowledge, this is the first public dataset which contains samples with sequential dependence of click and conversion labels for CVR modeling.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

==> ch_problem_overview.tex <==
\section{Characters of CTR and CVR modeling}\label{sec:ctr_cvr_model}

In this section, we first overview the formulation of CTR and CVR modeling. 
We then introduce the characteristics of data as well as arising challenges. 
Finally, we discuss the shortcomings of conventional modeling approach.  

For the sake of simplicity， we limit ourself in the area of advertising in e-commerce industry.
Discussions here are also applicable in similar scenarios such as recommendation system.  

%1. 介绍CTR、CVR问题的特点和挑战,数学化定义
%   p(z=1,y=1|x) = p(y=1|x) * p(z=1|y=1,x)
%   target、观测集、inference集
%2. 介绍数据的特点、分布，带来的挑战 
%3. 介绍典型的解法：
%   1）单CTR/CVR建模，然后pCTR*pCVR，问题：scale match问题
%   2）直接建模pCTCVR，问题：没有利用domain knowledge：pCTCVR目标过于稀疏，分解有助于降低复杂度

%\subsection{Problem Definition}

\subsection{Sample generation for CTR and CVR modeling}
Let's check carefully the sample generation process for both CTR and CVR modeling. 
\begin{itemize}
\item user U visited taobao.com and the recommender selected and displayed ten ads to U, which logged as ten impressions in system data, 
\item U clicked two interested ads A and B, hence marked the two related impressions with positive click label and other eight impressions with negative click label, 
\item U purchased ad A pointed goods, again marked ad A related impression with positive conversion label and the other clicked impression with negative conversion label. 
\end{itemize}
In other words, samples are generated following the \textit{impression $\rightarrow$ click $\rightarrow$ conversion} paradigm.

Mathematically, impression is featured as vector $X \in R^d$. $X$ is usually one-hot or multi-hot vector with dimension d scales up to $10^6 \sim 10^9$.
Click and conversion label is denoted by y and z respectively.       
\[
y = \begin{cases}
  1, & \text{click,} \\
  0, & \text{no click.}
\end{cases}
z = \begin{cases}
  1, & \text{conversion,} \\
  0, & \text{no conversion.}
\end{cases}
\]

Denote $S_X=\{X_i\}|_{i=1}^n$ to be all the impressions and $S_X^+=\{X_j|y_i=1\}|_{j=1}^m$ as the clicked impressions. 
Dataset for conventional CTR modeling is $\{X_i,y_i\}|_{i=1}^n, X_i \in S_X$ and dataset for conventional CVR modeling is $\{X_j,z_j\}|_{j=1}^m, X_j \in S_X^+$.

\subsection{Theoretical Analysis of CTR and CVR modeling} \label{sec:theo}
Given impression X, the probability of click and conversion event occurred is defined as: 
\begin{equation} \label{math:pctcvr}
\begin{split}
\textsl{pCTCVR} &= p(y=1, z=1|X) \\
                &= p(y=1|X) \times p(z=1|y=1,X) \\
                &= \textsl{pCTR} \times \textsl{pCVR} 
\end{split}
\end{equation}

While it is possible to model $p(y=1, z=1|X)$ directly, the decomposition of (\ref{math:pctcvr}) has several advantages.
\begin{itemize}
\item It makes use of the domain knowledge about the user behavior paradigm and split the probability into two steps of \textit{p(impression $\rightarrow$ click)} and \textit{p(click $\rightarrow$ conversion)}, which is promising to perform better than without it.      
\item It may predict more accurately on users with few or no conversions and a reasonable amount clicks because in that case \textsl{pCTR} still provide some information. [TODO:ref delayedConv]     
\end{itemize}

      
 
\subsection{Challenges on CVR modeling}
Through CVR modeling is quite similar to CTR modeling, several task specific problems make it rather challengeable and should pay more efforts on. 
We report three relatively serious problems encountered in industrial practice.       
\begin{itemize}
\item \textit{Delayed feedback problem}. As is discussed by previous work [TODO:ref] that in  some scenarios conversion event will be observed after a long delay. For example, [TODO: delayConv] shows about $50\%$ of conversions are occurred after 24 hours in their system. However, similar to Yahoo RMX exchange system[TODO:ref], the degree of conversion delay in our system is slightly acceptable.    
\item \textit{Data sparsity problem}. Practically both click and conversion are rarely occurred event, with traditional probability of CTR to be of order $10^{-2}$ and CVR of order $10^{-3}$. This causes the data collected for training CVR model is much less than CTR task. Taken into consideration of the high nonlinearity of CVR task, data sparsity makes it rather tough for CVR modeling.         	
\item \textit{Sample bias problem}. As discussed above, samples for CVR modeling are collected from post-click setting. That is, preceding click event acts as a hidden sampler which generates training data $S_X^+$ for CVR task from whole impression set $S_X$.  
    While at inference stage, it is required to predict the whole impression set $S_X$.  
    As click event is rare and is more likely to occur for impressions with high click probability, causing the sampling for CVR task to be uneven w.r.t. original impression distribution. 
    In other words, there lies a sample bias between CVR training and inference.          
\end{itemize}

Several approaches have been proposed to solve the \textit{delayed feedback problem} and \textit{Data sparsity problem} for CVR modeling.    
However,to the best of our knowledge, this is the first work which carefully discusses  \textit{sample bias problem} in the scenario of CVR modeling. 
In the following section, we will introduce in detail about our proposed approach, which jointly models CTR and CVR via a multi-task deep learning network, bringing a cute solution which can help overcoming both the \textit{data sparsity} and \textit{sample bias} problem.    
In this paper, we make no effort to solve the \textit{delayed feedback problem} and leave it for future work.  






==> mtl_intro.bak.tex <==
\section{Introduction}
%介绍预估的应用背景
Predicting user's click or conversion probability is an essential task for ranking system in industrial applications, such as online advertising, recommendation etc.  Estimating these probabilities accurately is critical for these businesses worth hundreds of billions of dollars~\cite{jindeep}. 

%介绍典型的应用方法
In many systems, such as display advertising in e-commerce, user behavior usually follows the sequential pattern of (impression, click, conversion). In this scenario, CTR modeling refers to prediction of post-view click-through rate, i.e., $\textit{pCTR} = p(click|impression)$ and CVR modeling refers to prediction of post-click conversion rate, i.e., $\textit{pCVR} = p(conversion|click,impression)$. Another derived probability is \textit{pCTCVR}, which refers to post-view click-through and conversion rate. It can be calculated as $\textit{pCTR} \times \textit{pCVR}$.
  
Practically, predicted probabilities of \textit{pCTR},\textit{pCVR} and \textit{pCTCVR} play fundamental roles in the ranking system in these applications. For example: i) in CPC(cost-per-click) advertising~\cite{ftrl}, $\textit{rank-score}$ = $\textit{pCTR}\times\textit{bid-price}$, ii) in OCPC(optimized-cost-per-click) advertising~\cite{zhu2017optimized}, $\textit{rank-score}$ = $\textit{pCTR}\times\textit{optimized-bid-price}$, where \textit{optimized-bid-price}=$f(\textit{bid-price, pCTR, pCVR})$, iii) in recommendation system, $\textit{rank-score}$ = $\textit{pCTCVR}\times\textit{item-price}$~\cite{liu2017cascade,yan2017optimizing}.

\begin{figure}[!t]
\centering
\includegraphics[height=32mm ]{figures/path-label-2.pdf}
\caption{{Illustration of sample selection bias problem for the CVR modeling. Training space is composed of clicked impressions. It is only part of the inference space which is composed of all impressions.}}
\label{fig:pl}
\end{figure}

There has been significant work in the literature on CTR modeling in the context of advertising and recommendation~\cite{ftrl,MLR,FbCtr,widedeep,din}, but relatively little on CVR modeling~\cite{delayConv,ecvr,pcvr}. In general, most industrial applications employ similar techniques developed in CTR task to build CVR model, which results in the CVR-task-specific challenges. In the paper, we focus on solving the \textit{sample selection bias problem}, as illustrated in Fig\ref{fig:pl} and \textit{data sparsity problem}, which are two particularly critical problems in practice. 
%However, CVR modeling has encountered many task-specific challenges, among which we report two particularly critical problems in practice.  
%\begin{itemize}
%\item \textit{Sample selection bias problem}. 
%   In the \textit{impression $\rightarrow$ click $\rightarrow$ conversion} paradigm, conventional CVR models are trained on dataset consisting of clicked impressions, while used to predict on the full set of impressions, as illustrated in Fig.\ref{fig:pl}.
%\item \textit{Data sparsity problem}. 
%   Due to the rare occurrence of click event, data gathered for training CVR model is generally 2-3 orders of magnitude less than CTR task. Sparsity of training data makes CVR model fitting to be rather difficult. 
%\end{itemize}

we propose a novelly designed full-path prediction model (FPPM) to jointly learn CTR and CVR. The FPPM defines the path-label as $(click, conversion)$ and directly models $p((click, conversion)|impression)$ over the entire input space and outputs $\textit{pCTR}$, $\textit{pCVR}$ and $\textit{pCTCVR}$ at the same time. The design of our model can effectively skip the \textit{sample selection bias problem} occured in the conventional CVR modeling. Besides, by sharing the feature representation of CTR and CVR using mutil-task learning, the FPPM provides a classical approach to solve the \textit{data sparsity problem}~\cite{TLsurver}. Since it is the first work to jointly learn CTR and CVR, there are no public datasets provided before. We collect and release the traffic logs from a productive display advertising system for the future research\footnote[1]{see: www.www}. Careful experiments are conducted to demonstrate the effectiveness of the proposed approach.

%On the other hand, we do expect conversion to be an enhanced click signal to improve CTR modeling. A simple observation is that clicks followed by conversions are merely possible to be robot generated. However, experimentally we observe similar performance of CTR network of FPPM compared with individually trained CTR model. 
%This might attribute to the preprocessed anti-spamming on our dataset. 
%We leave it for future research and focus mainly on the improvement of CVR modeling in the rest of the paper. 

The rest of the paper is organized as follows: section 2 gives formulation and evolution of the proposed approach. We conduct experiments in section 3 and give a conclusion in section 4. 






  



            

%% qingli's version
\begin{comment}

%从用户角度引出预估任务，强调其重要性
As the development of ranking system, one of the important trend is different items are showed for different people in order to enhance the user experience and the business value of the traffic~\cite{jindeep}. The key of this technology is to bring in the prediction model as the main factor of the ranking. Different prediction models is designed carefullly to meet the need of user and system.

In most ranking systems, user's behavior follows the certain pattern, which can be represented as \textit{impression $\rightarrow$ click $\rightarrow$ conversion}. Combined with the pattern, we give an overview of the classical prediction models in the table 1. It is worth mentioning that the CCR model is rarely trained individually, since it can be calculated from $\textit{pCCR} = \textit{pCTR}*\textit{pCVR}$. Below is the list of several famous systems and the introduction of how to use these prediction models in the systems:
\begin{itemize}
\item \textit{Ranking in online advertising system}. 
   %$\textit{pCTR}$ and $\textit{pCVR}$ are key factors in ranking score function. 
   Different payment settings of advertising system designs different ranking score functions, for example: 
   i) in CPC(cost-per-click) $\textit{score}$ = $\textit{pCTR}\times\textit{bid-price}$, 
   ii) in CPA(cost-per-conversion) $\textit{score}$ = $\textit{pCCR}\times\textit{bid-price}$, 
   iii) in OCPC(optimized-cost-per-click) $\textit{score}$ = $\textit{pCTR}\times\textit{optimized-bid-price}= \textit{pCTR}\times f(\textit{bid-price, pCTR, pCVR})$, where $f(\cdot)$ is an algorithm based model~\cite{zhu2017optimized}. 
\item \textit{Reranking in recommendation system}. In e-commerce platform, recommended items are reranked for the sake of total GMV(gross-merchandise-volume). A commonly used rerank $\textit{score}$ = $\textit{pCTCVR}\times\textit{item-price}$~\cite{liu2010personalized}. [TODO: wrong ref]
 \end{itemize}

\begin{table}[!t]
  \caption{{\small Different prediction models}}
  \label{tab:hint}
\centering{\footnotesize
 \centerline {\begin{tabular}{lcc}
 \toprule
model & meaning & formula\\
\midrule
CTR & post-view click-through rate & $\textit{pCTR} = p(click|impression)$ \\
CVR & post-click conversion rate & $\textit{pCVR} = p(conversion|click,impression)$ \\
CCR & post-view click and conversion rate & $\textit{pCVR} = p(click,conversion|impression)$ \\
\bottomrule
\end{tabular}}}
\end{table}


Given the significance of these prediction model in the ranking system, much work in the literature on CTR modeling has been done in the context of advertising and recommendation~\cite{ftrl,MLR,FbCtr,widedeep,din}, while relatively little are promoted on CVR modeling~\cite{delayConv,ecvr,pcvr}. 
Most industrial applications employ similar techniques developed in CTR task to build CVR models by ignoring the specific properties of the CVR model. In fact, the CVR model has many task-specific challenges, among which we introduce two particularly critical problems in practice.  
%In this paper, we report two critical challenges that we face in CVR modeling practically.
\begin{itemize}
\item \textit{Sample selection bias problem}. 
   In the \textit{impression $\rightarrow$ click $\rightarrow$ conversion} paradigm, conventional CVR models are trained on dataset consisting of clicked impressions, while used to predict on the full set of impressions, as illustrated in Fig.\ref{fig:pl}.
   
\item \textit{Data sparsity problem}. 
   Due to the rare occurrence of click event, data gathered for training CVR model is generally 2-3 orders of magnitude less than CTR task. 
   %While it is is a common practice to train CTR and CVR models on the same (or with most of features the same) high dimensional discrete feature space which is designed manually with lots of engineering effort. 
   Sparsity of training data makes CVR model fitting to be rather difficult. 
\end{itemize}

In this paper, we propose a path-label learning framework to jointly model CTR and CVR. The main contribution of the framework is :
\begin{itemize}
\item \textit{unbiased CVR model by jointly modelling.} The framework provides a new way by directly modeling $p(click \rightarrow conversion|impression)$ over the entire input space and outputs $\textit{pCTR}$, $\textit{pCVR}$ and $\textit{pCCR}$ simultaneously. To the best of our knowledge, this is the first work in this field that jointly models CTR and CVR.
%This enables FPPM to skip the \textit{sample selection bias problem} for CVR modeling.  
\item \textit{Feature representation transfer learning.} Part of the features in CTR and CVR network are shared together using multi-task learning~\cite{baxter1997bayesian} to solve the data sparsity problem in the CVR model~\cite{TLsurver}. 
\item \textit{Public dataset for further research.}We collect traffic logs from a productive display advertising system for this work since there is no related public datasets before. To help the community for future research, we release our collected dataset\footnote[1]{see: www.www}.   
%Careful experiments are conducted and demonstrates the effectiveness of the proposed approach. 
\end{itemize}


\begin{figure}[!t]
\centering
\includegraphics[height=32mm ]{figures/path-label-2.pdf}
\caption{{Illustration of sample selection bias problem for CVR modeling task. Training space is composed of clicked impressions. It is only part of the inference space which is composed of all impressions.}}
\label{fig:pl}
\end{figure}

    
The rest of the paper is organized as follows: section 2 gives detail of the proposed framework. The experiment and conclude are described in section 3 and 4. 

\end{comment}














   


%介绍预估的应用背景
%Predicting users' click or conversion probability is an essential task for ranking system in industrial applications, such as online advertising, recommendation etc.  
%Estimating these probabilities accurately is critical for these businesses which valued hundreds of billions of dollars~\cite{jindeep}. 
%如advertising system，recommender system等，这是一个hundreds of billions business



%经典方法和问题的介绍

%我们框架的大致方法和贡献点

%论文结构

%介绍典型的应用方法
 %In many system, such as advertising system in taobao, the largest e-commence site in China, user interface is designed according to the habits of web users. 
 %It follows a impression $\rightarrow$ click $\rightarrow$ conversion paradigm, that is, users first click viewed items into the item detail page and then  decide to purchase if satisfied.  

%In many systems, such as display advertising in e-commerce,  user behavior usually follow a \textit{impression $\rightarrow$ click $\rightarrow$ conversion} paradigm.      
%In this scenario, CTR modeling refers to prediction of post-view click-through rate, i.e., $\textit{pCTR} = p(click|impression)$ and CVR modeling refers to prediction of post-click conversion rate, i.e., $\textit{pCVR} = p(conversion|click,impression)$.

%预估目前的背景和应用

%In this scenario, CTR and CVR prediction tasks are formalized as: i) prediction of post-view click-through rate, i.e., $\textit{pCTR} = p(click|impression)$, ii) prediction of post-click conversion rate, i.e., $\textit{pCVR} = p(conversion|click,impression)$.
%In this scenario, CTR and CVR prediction tasks are formalized as: i) CTR task aims to predict post-view click-through rate, i.e., $\textit{pCTR} = p(click|impression)$, ii) CVR task aims to predict post-click conversion rate, i.e., $\textit{pCVR} = p(conversion|click,impression)$.
%\begin{itemize}
%\item CTR task aims to predict post-view click-through rate, i.e., $\textit{pCTR} = p(click|impression)$, 
%\item CVR task aims to predict post-click conversion rate, i.e., $\textit{pCVR} = p(conversion|click,impression)$.     
%\end{itemize}
%Another derived but important probability \textit{pCTCVR}, which refers to  post-view click-through and conversion rate, is calculated as $\textit{pCTR} \times \textit{pCVR}$.
%Note that, there is a different CVR task which focuses on predicting post-view conversion rate. It is beyond the scope of this paper. 
  
%Practically, \textit{pCTR},\textit{pCVR} and \textit{pCTCVR} play fundamental roles in the ranking system in different applications.
%Practically, predicted probabilities of \textit{pCTR},\textit{pCVR} and \textit{pCTCVR} play fundamental roles in the ranking system in these applications. For example: i) in CPC(cost-per-click) advertising~\cite{ftrl}, $\textit{rank-score}$ = $\textit{pCTR}\times\textit{bid-price}$, ii) in OCPC(optimized-cost-per-click) advertising~\cite{zhu2017optimized}, $\textit{rank-score}$ = $\textit{pCTR}\times\textit{optimized-bid-price}$, where \textit{optimized-bid-price}=$f(\textit{bid-price, pCTR, pCVR})$, iii) in recommendation system, $\textit{rank-score}$ = $\textit{pCTCVR}\times\textit{item-price}$ [TODO: add ref]. 
\begin{comment}
\begin{itemize}
\item \textit{Ranking in online advertising system}. 
   %$\textit{pCTR}$ and $\textit{pCVR}$ are key factors in ranking score function. 
   Different payment settings of advertising system designs different ranking score functions, for example: 
   i) in CPC(cost-per-click) $\textit{score}$ = $\textit{pCTR}\times\textit{bid-price}$, 
   ii) in CPA(cost-per-conversion) $\textit{score}$ = $\textit{pCTCVR}\times\textit{bid-price}$, 
   iii) in OCPC(optimized-cost-per-click) $\textit{score}$ = $\textit{pCTR}\times\textit{optimized-bid-price}= \textit{pCTR}\times f(\textit{bid-price, pCTR, pCVR})$, where $f(\cdot)$ is an algorithm based model~\cite{zhu2017optimized}. 
\item \textit{Reranking in recommendation system}. In e-commerce platform, recommended items are reranked for the sake of total GMV(gross-merchandise-volume). A commonly used rerank $\textit{score}$ = $\textit{pCTCVR}\times\textit{item-price}$~\cite{liu2010personalized}. [TODO: wrong ref]
 \end{itemize}
\end{comment}



   %This bias decreases the   
   %Taking into consideration that click events are rarely occurred and with click probability varies over different regions, it causes the drift of distribution of training samples from truly underling distribution, where inference samples are drawn from.   
   %Taking into consideration that click events are rarely occurred, to say nothing of the click probability varies in different regions, it will cause the distribution of training set to be shifted from truly underling distribution.


%% simple version
%In this paper, we propose a novelly designed multi-task deep learning network (FPPM) to jointly model CTR and CVR. %, as illustrated in Fig.\ref{fig:mtl}.



%On one hand, FPPM finds a new way by directly modeling $p(click \rightarrow conversion|impression)$ over the entire input space and outputs $\textit{pCTR}$, $\textit{pCVR}$ and $\textit{pCTCVR}$ at the same time. 
%This enables FPPM to skip the \textit{sample selection bias problem} for CVR modeling.  
%Besides, embedding parameters of same features for CTR and CVR network in FPPM are shared together, playing the role of feature representation transfer learning~\cite{TLsurver}. 
%It is helpful for improving the convergence of CVR network with sparse data.
%On the other hand, we do expect conversion to be an enhanced click signal to improve CTR modeling. 
%A simple observation is that clicks followed by conversions are merely possible to be robot generated. 
%However, experimentally we observe similar performance of CTR network of FPPM compared with individually trained CTR model. 
%This might attribute to the preprocessed anti-spamming on our dataset. 
%We leave it for future research and focus mainly on the improvement of CVR modeling in the rest of the paper.

%% full version
\begin{comment}  
In this paper, we propose a novelly designed multi-task deep learning network (FPPM) to jointly model CTR and CVR, as illustrated in Fig.\ref{fig:mtl}.
On one hand, co-training of multi tasks in FPPM brings the profit to assist CVR task to tackle the challenges above mentioned. %while with little side-effect on the performance of CTR model itself.  
Unlike conventional approaches which consider click and conversion as two separate scalar labels, here we treat them as an united \textit{path-label}. 
That is, our approach directly models $p(click \rightarrow conversion|impression)$ and outputs $\textit{pCTR}$, $\textit{pCVR}$ as well as $\textit{pCTCVR}$ at the same time. 
Samples are fed into trainer with format $\{ \textit{impression : (click,conversion)} \}$. 
In this manner, FPPM-CVR network is actually trained on the entire input space, accompanied by FPPM-CTR and FPPM-CTCVR network, skipping the \textit{sample bias problem}.
Besides, embedding parameters of same features in FPPM-CTR and FPPM-CVR network are shared together, playing the role of feature representation transfer learning~\cite{TLsurver}. This is helpful for improving the convergence of CVR network if trained  with sparse data individually.       
On the other hand, we do expect conversion label to be an enhanced click signal to help CTR modeling. 
A simple observation is that clicks followed by conversions are merely possible to be robot generated. 
However, experimentally we observe almost the same performance of FPPM-CTR model compared with individually trained CTR model. 
This may be due to the dataset used in our experiments has beed processed after anti-spamming. 
We leave it for future research and focus mainly on the improvement of CVR modeling in the rest of the paper.
\end{comment}


%We summarize the contributions of this paper as follows:
%\begin{itemize}
%\item we study and propose the \textit{sample bias problem} for CVR modeling,
%\item we design a novel multi-task deep learning network which jointly trains FPPM-CTR and FPPM-CVR models and achieves  significant improvement on the CVR task compared with individually trained CVR models,   
%\item we release the first CTR-CVR co-training dataset collected from productive advertising system.
%\end{itemize}

                            


  

%介绍相关的建模思路以及存在的问题，本文的重点
%There has been significant work in the literature on modeling clicks in the context of search advertising [5, 11] and display advertising [1, 2], but relatively little on conversion prediction [16]. This paper deals with the problem of conversion prediction and more specially with post-click conversions, these conversions that can be attributed to a preceding click.
%There has been significant work in the literature on CTR modeling in the context of advertising and recommendation~\cite{ftrl,MLR,FbCtr,widedeep,din}, but relatively little on CVR modeling~\cite{ecvr,pcvr}. 
%In general, most industrial applications employ similar techniques developed in CTR task to build CVR models, 
%By analogy with the CTR task which trains model on \textit{impression $\rightarrow$ click} samples, 
%CVR task trains model on \textit{click $\rightarrow$ conversion} samples of which clicked impressions serve as samples with/without conversions as positive/negative labels[TODO:ref].
%with additional efforts payed on handling CVR task specific issues. 
%We summarize two main concerns discussed in the literature : 
%\begin{itemize}
%\item\textit{delayed feedback problem} which deals with the delayed conversion label~\cite{chapelle2014modeling}, 
%\item\textit{data sparsity/unbalance problem} which is caused by rare occurrence of conversion event~\cite{lee2012estimating}.
%\end{itemize}
 %with unbalanced learning methods such as sampling[TODO:ref].
%However, to the best of our knowledge, no work in the literature tries to solve the \textit{sample bias problem} of CVR modeling. 
%That is, training on sample space with clicked impressions while inferencing on the whole impression space, as illustrated in Fig.\ref{fig:pl}.



%To better understand the sample bias problem, let's check carefully the sample generation process: i) user U visited taobao.com and the recommender selected and displayed ten items to U, which logged as ten impressions in system data, ii) U clicked two interested items A and B, hence marked the two related impressions with positive click label and other eight impressions with negative click label, iii) U purchased item A, again marked item A related impression with positive conversion label and the other clicked impression with negative conversion label. 
%Viewing the process from a whole, samples were collected along the generative path of \textit{impression $\rightarrow$ click $\rightarrow$ conversion}. 
%Click event affects the sample distribution of CVR task. 
% 这个点留到正文中具体展开
%Intuitively, CVR is somewhat relevant to CTR, because users click or purchase items may both originated to the interest in the viewed items while are merely possible to purchase items without firstly clicking them. 
%Fig. [TODO:fig2] demonstrates the relevance of CTR and CVR in our system. 
%In [TODO:ref:Post-Click Conversion Modeling and Analysis], authors also conduct experiments to check the relationship of CTR and CVR modeling and report observations of the relevant evidence.         
%Preceding click event acts as a hidden sampler which generates training data for CVR task from whole impression distribution.  
%Unless probability variables of $\textit{pCTR}$ and $\textit{pCVR}$ are conditionally independent w.r.t. impression event, which is obviously not true and is demonstrated in Sec. 3, click event sampler will has no influence on CVR task. 
%In other words, individually modeling CVR without taking into consideration of CTR factor will brings sample bias. %$p$(conversion$|$click;impression).
%As click itself is also a rarely occurred event, traditionally with probability of $10^{-2}$, only a small portion of the whole impression space is explored for training CVR model, leaving the huge difficulty for inferencing on the whole impression space. Hence,



  


==> mtl_relatedwork.tex <==
\section{Related work}


%介绍multi-label的定义和方法,以及我们的工作
{\bfseries Multi-label Learning}. In the task of supervised Learning, the goal is to learn a function \textit{f : X $\rightarrow$ Y}, \textit{X} denotes the d-dimensional instance space and \textit{Y} denotes the k-dimensional label space. If \textit{k $>$ 1}, we call it a multi-label learning task. Multi-label learning algorithms mainly devided into algorithm adaptation and problem transformation methods~\cite{zhang2014review}. In our task, the predicted label is 2-dimension including both click and conversion. We use the relation of click and conversion as the prior knowledge to model the whole transformation process, which is one kind of algorithm adaptation~\cite{xu2016robust}.

%介绍multi-task的定义和方法，以及我们的工作
{\bfseries Multi-task Learning}. In multi-task learning, multiple tasks is learned simultaneously by sharing representation knowledge between tasks. Higher prediction accuracy is expected in multi-task learning than individual trained tasks. There are two patterns of sharing in Multi-task Learning, hard parameter sharing~\cite{baxter1997bayesian} and soft parameter sharing~\cite{duong2015low}. Tasks using hard parameter sharing share the same parameter between all tasks, while soft parameter sharing on the other hand, can have their own parameter for each task by using regularization to make the parameters be similar~\cite{yang2016trace}. In the paper, we try both methods to jointly model the Click Through Rate and Converation Rate prediction via Multi-task learning.

%介绍Unbiased Learning的定义和方法，以及我们的工作
{\bfseries Unbiased Learning}. The difference of distribution between training set and inference set usually result in bias problem. The classical method for unbiased learning is sampling to simulate the distribution of inference set~\cite{zoghi2017online}. Since the real distribution of inference set is unkown, the strategy of sampling need to keep tuning according to the online effect, which brings the great challendge for online. ~\cite{zhang2016bid} provides another method by giving an adjusted weight for sample using its auction probability. Different from the above work, our work provides a method in unbiased learning by modelling the whole click and conversion process.

%整体介绍我们的工作。
Our work take both click and conversion as label to model the Click Through Rate and Converation Rate prediction. Meanwhile, by sharing the embedding representation, the prediction accuracy is highly improved compared the individual prediction Model. The whole work can be seen as a multi-label learning or a multi-task learning. The end-to-end modeling can also regard as an unbiased learning framework, which solve the sample bias problem for Converation Rate Model.
